Schema2QA: High-Quality and Low-Cost Q&A Agents for the Structured Web

Building a question-answering agent currently requires large annotated datasets, which are prohibitively expensive. This paper proposes Schema2QA, an open-source toolkit that can generate a Q&A system from a database schema augmented with a few annotations for each field. The key concept is to cover the space of possible compound queries on the database with a large number of in-domain questions synthesized with the help of a corpus of generic query templates. The synthesized data and a small paraphrase set are used to train a novel neural network based on the BERT pretrained model. We use Schema2QA to generate Q&A systems for five Schema.org domains, restaurants, people, movies, books and music, and obtain an overall accuracy between 64% and 75% on crowdsourced questions for these domains. Once annotations and paraphrases are obtained for a Schema.org schema, no additional manual effort is needed to create a Q&A agent for any website that uses the same schema. Furthermore, we demonstrate that learning can be transferred from the restaurant to the hotel domain, obtaining a 64% accuracy on crowdsourced questions with no manual effort. Schema2QA achieves an accuracy of 60% on popular restaurant questions that can be answered using Schema.org. Its performance is comparable to Google Assistant, 7% lower than Siri, and 15% higher than Alexa. It outperforms all these assistants by at least 18% on more complex, long-tail questions.

==> sections/algorithm.tex <==
%!TEX root = ../paper.tex
\section{Training Data Synthesis}
\label{sec:algorithm}
Previous work by Wang et al.~\cite{overnight} introduced the
idea of synthesizing data from domain-independent templates,
combined with domain-specific \textit{canonical forms} associated
with each table and field. Yet, their simplistic template set generates low-quality sentences that are unsuitable for training. 
%Subsequent work shows that allowing developers supply domain-specific templates can generate higher quality synthetic sentences, which can be included with a small amount of paraphrase data for effective training~\cite{geniepldi19}.  
We claim that a carefully tuned set of templates can improve the quality
of the synthesized data. In this section, we propose the \SQA templates, and the associated set of canonical forms. Ours is the first template
model for question answering that synthesizes varied, complex, yet still natural questions.

\iffalse
We propose classifying canonical forms into more POS categories\footnote{The abbreviations
are based on POS tags from the Penn Treebank tagset.} 
and use curated generic templates for each POS category to synthesize more varied and useful training sets. 
%\webqa applies an off-the-shelf part-of-speech tagger to identify the POS tag of generated canonical forms.
\fi

\begin{table*}
\caption{Examples of Generic Templates used by \webqa to Generate Training Data}
\vspace{-1em}
\small
\begin{tabular}{p{10cm}|p{6cm}}
\toprule
{\bf Template} & {\bf Example Sentence}\\
\midrule
projection $:=$ ``the'' $p : \text{prop}$ ``of'' $t : \text{table}$ & ``the rating of Panda Express''\\
\hline
table $:=$ $t : \text{table}$ ``that have'' $p : \text{prop}$ ``more than'' $v : \text{value} \Rightarrow t, p \ge v$ & ``restaurants that have rating more than 4''\\
\hline
table $:=$ $t : \text{table}$ ``with the highest'' $p : \text{prop} \Rightarrow \left(\texttt{sort}~~p~~\texttt{desc of }t\right)[1]$ & ``restaurants with the highest rating''\\
\hline
question $:=$ ``how far is'' $t : \text{table} \Rightarrow \texttt{compute}~~\text{distance}\left(\textit{geo}, \texttt{here}\right)~~\texttt{of}~~t$ & ``how far is Starbucks?''\\
\bottomrule
\end{tabular}
\label{table:template-examples}
\end{table*}

\subsection{Template-Based Synthesis}

To synthesize data for the neural semantic parser, \webqa uses a template-based 
algorithm with a curated set of domain-independent templates. 
The pipeline to get the final training examples is shown in Figure~\ref{fig:genie}.

\begin{figure}[h]
\centering
\includegraphics[width=0.9\linewidth]{./figures/genie-diagram.pdf}
\caption[]{Training data synthesis pipeline.}
\label{fig:genie}
\Description{}
\end{figure}


Unlike previous work~\cite{geniepldi19} replying on hand-written domain-specific templates,
\webqa uses \textit{canonical forms} for each table and field in the domain,
which can be generated automatically as in \NLSchema.
Canonical forms represent all the ways the field is referred to in natural language. Each canonical form is also annotated with its part-of-speech (POS) tag.

The \textit{templates} are production rules mapping the grammar of natural language to a \textit{semantic function} that produces the corresponding code. 
Formally, a template is expressed as:
\begin{align*}
\textit{nt} := \left[v : \textit{nt}~~\vert~~\text{literal}\right]^+ \Rightarrow \textit{sf}
\end{align*}
The non-terminal \textit{nt} is produced by expanding the terminals and non-terminals
on the right-hand side of the $:=$ sign.
The bound variables $v$ are used by the semantic function \textit{sf} to produce the corresponding code.
\webqa expands the templates by substituting the non-terminals with the previously generated
derivations and applying the semantic function. The expansion continues recursively, up to a configurable depth. 

Templates are written by hand, and map natural language compositional constructs to formal language operators.
Many sentences can be covered with \webtalk templates, such as:
\begin{tabbing}
12345678901234\=1234\=\kill
\>table $:=$ $t : \text{table}$ ``that'' $p : \text{vb}$ $v : \text{value}$ \\
\>\>$\Rightarrow t, \text{contains}(p, v)$
\end{tabbing}
This template can generate ``hotel that offers free parking''.
In this case, the table is ``Hotel'', and the field is ``amenityFeature'' with has canonical form ``offers'' in the VB (verb) category.
Templates rely on the type system to form sentences that are meaningful and map to correct queries.
%For example, in the following template, only fields of comparable type can be used:
%\begin{tabbing}
%123\=1234\=\kill
%\>table $:=$ $t : \text{table}$ ``whose'' $p : \text{npp}$ ``is less than'' $v : \text{value}$ \\
%\>\>$\Rightarrow t, p \le v$
%\end{tabbing}
%The template would generate ``restaurants whose rating is less than 3'', but it would not generate
%``restaurants whose cuisine is less than Italian'', as the latter would not typecheck.
Typing is also used to automatically add computation, aggregation and sorting.

A small subset of synthesized data is paraphrased by crowd workers to provide more variety.
Then both the synthetic and paraphrased set is augmented by replacing parameters with 
the actual values in \NLSchema knowledge base. 
This allows us to expose more real values to the neural network
to learn how they match to different properties. 
Finally, the augmented dataset will be used for training our semantic parser.

\subsection{Templates For Question Answering}
Previous work designed a set of templates that primarily focused on joins, and used a limited set of POS tags~\cite{overnight}. Empirically, we observed that the most common useful complex queries use few joins, but use many filters, as well as argmin/argmax. We designed our set of templates to match the questions we gathered during the development of \webqa. Here we describe the rationale.

Overall, \webqa includes 512 hand-curated templates. 
Shown in Table~\ref{table:template-examples} are some examples of templates and generated sentences:  
a projection of a field of the table, a comparison filter,
an argmax aggregation operation, and a computed field.

\paragraph{Filters.}
Table~\ref{table:comparison}
shows that filters are used in many meaningful queries where all 10 examples use at least one filter. For this reason, 208 \webqa templates (41\%) are dedicated to understanding filters. 
We observed that filters for the same field can correspond to different grammar categories. 
We found that there are six grammar categories that cover most of the ways properties are queried. 

Four of the six categories correspond to POS categories of the canonical forms of a field: \textit{noun-phrase for property field (prop)}, \textit{noun-phrase for identity field (identity)}, \textit{verb-phrase field (verb)}, \textit{passive verb phrase field (passive\_verb)}. For example, the ``alumniOf'' field of ``Person'' has identity form ``alumni of'' (``who is an alumni of X?'') and verb form ``graduated from'' (``who graduated from X?''); similarly, the ``author'' field of ``Review'' has prop form ``author'' (``what review has author John Doe?'') and passive\_verb form ``written by'' (``what review is written by John Doe?'').

We observed that for some fields, just the mention of their value is sufficient to identify the field used. We introduce two more kinds of annotations: \textit{noun-phrase for value (noun)} and \textit{adjective-phrase for value (adj)}. For example, the field ``servesCuisine'' in the ``Restaurant'' class is annotated adj, because it can be used implicitly in ``show me Mexican restaurants''.

We also observed that in English, filters can involve a phrase before and a phrase after the value. For this reason, we allow canonical forms to use ``\#'' to indicate where to put the value.
For example, one of the canonical forms of the ``servesCuisine'' field in the ``Restaurant'' class (Fig.~\ref{fig:example-schema}) has verb form ``serves \# cuisine''. This allows
\webqa to generate sentences of the form ``restaurants that serve Italian cuisine'', where the value ``Italian'' is in between ``serves'' and ``cuisine''.

\paragraph{Combining operators.}
Previous work used at most one target language operator in each template, but we noted that multiple \DBTalk operators can be combined to compose common natural language concepts. For example, \webqa includes 94 templates for \textit{argmax} and \textit{argmin} operations. These are templates that combine the sort and index operators to select the minimum or maximum row in the table.
The argmax template is used to understand questions that choose the most highly rated restaurant (Table~\ref{table:comparison}).

\paragraph{Type-based templates.}
We noted that certain fields or types can generalize across many different domains, so we include type-specific templates in \webqa. For example, all tables that use the ``geo'' field can make use of ``how far'' (Table~\ref{table:comparison}) and ``nearest'' templates to ask location queries. This design is possible because we use a strong type system.

\iffalse
\webqa puts particular emphasis on generating understandable and varied questions for them.
Because filters are the hardest and most important feature of a query system, 41\% of \webqa are dedicated to them.  so  
\fi

\iffalse
To use \webqa, each field in the domain is annotated with a list of \textit{canonical forms}, which represent all the ways the field is referred to in natural language. Each canonical form is also annotated with its part-of-speech (POS) tag. The domain-independent templates in \webqa
make use of the canonical forms of the correct tag to generate sentences
that refer to each field. 
The canonical forms can be provided by domain expert or collected via crowdsourcing.

For example, the ``author'' field of the ``Review'' table might have canonical forms ``author'' and ``written by''. Given the domain-independent templates:
\begin{tabbing}
123\=1234\=\kill
\>table $:=$ $t : \text{table}$ ``whose'' $p : \text{nnp}$ ``is'' $v : \text{value}$\\
\>table $:=$ $t : \text{table}$ $p : \text{jj}$ $v : \text{value}$
\end{tabbing}
\webqa is able to generate ``reviews whose author is ...'' and ``reviews written by ...''. ``nnp'' is the category of noun-phrase canonical forms, and ``jj'' is the category of adjective phrases (incl. passive verbs).
\fi

\iffalse
\webqa makes use of \webtalk's native support for the Location type to understand ``where'' questions and ``how far'' (distance) questions.
These questions use the ``geo'' property, and are available in all tables that support that property.
\fi


\iffalse
These templates make use of the canonical forms, with their associated
POS tag. \webqa users provide the canonical forms and POS tags for the domain of interest.
\fi

\iffalse
\subsection{Part-of-Speech Categories}
\iffalse
\webqa uses a template-based method to synthesize a large training set mapping natural language
questions to \DBTalk queries. To do so, each property is annotated
with its \textit{canonical forms}: a list of short phrases that indicates
how the property and its value are referred to in natural language.
Each canonical form also indicates the part-of-speech it belongs to so they are used in natural language templates correctly.
\fi

Empirically, we identified 6 POS categories of canonical forms, which 
cover the most common ways people ask questions about a property of a subject.

The {\em noun-phrase for property field (NNP)}
tag denotes a noun phrase representing what a subject has. 
For example, ``reviews'' is a NNP canonical form for the ``review'' property; examples of generated sentences are ``show me the reviews of the restaurant?'' and ``which restaurant has more than 5 reviews?''.
Most properties defined in schema.org have at least one NNP canonical form.

The {\em noun-phrase for identity field (NNI)}
tag denotes a noun phrase representing what a subject is. 
For example, ``alumni of'' is a NNI canonical form for the ``alumniOf'' property of people; an example is ``who is an alumni of X university?''.

The {\em verb-phrase field (VB)} 
tag denotes a verb phrase representing what a subject does.
For example, ``serves'' is a VB canonical form for the ``servesCuisine'' property; an example is ``what restaurants serve tacos?''.

The {\em adjective-phrase field (JJ)}
tag denotes an adjective or passive verb. 
For example, ``rated'' is a JJ canonical form for the ``rating'' property; an example is  ``restaurants rated 4.5 or above''.
Similarly, the preposition ``by'' is a JJ canonical form for the ``author'' property of ``Review''; an example is ``show me reviews by Bob Smith''.

Additionally, in some cases the property is not explicit in the question, and the {\em value}
is sufficient to infer what property the query should use. Thus, we create two categories based on values:

The {\em noun-phrase for value (NNV)}
tag on the property denotes that the value of a property indicates what a subject is. 
For example, the property ``jobTitle'' is annotated NNV, and an example is ``who is a CEO?''.  The property ``jobTitle'' is implicit.

The {\em adjective-phrase for value (JJV)}
tag denotes that the value of a property is an adjective. 
For example, the property ``servesCuisine'' is annotated JJV, and an example is ``show me Mexican restaurants''. Here, the property ``servesCuisine'' is implicit.
\fi

\iffalse
\begin{table*}
\caption{Template Candidates used by \webqa to Generate Domain-Specific Templates}
\small
\begin{tabular}{p{8cm}|l|l}
\toprule
{\bf Template Candidates} & {\bf Positive Example Queries} & {\bf Negative Example Queries}\\
\midrule
table $:=$ $v : \text{value}$ $t : \text{table}$ & ``Mexican restaurants'' & ``4.5 hotels''\\
\hline
table $:=$ $t : \text{table}$ ``in'' $v : \text{value}$ & ``hotels in Florida'' & ``restaurants in Mexican ''\\
\hline
table $:=$ $t : \text{table}$ ``with'' $v : \text{value}$ & ``hotels with fitness center'' & ``restaurants with Mexican''\\
\hline
table $:=$ $t : \text{table}$ ``containing'' $v : \text{value}$ & ``hotels containing fitness center'' & ``restaurants containing Mexican''\\
\hline
table $:=$ $t : \text{table}$ $p : \text{(vb | vb\_prefix)}$ $v : \text{value}$ & ``person works for Google'' & ``restaurants serves Mexican''\\
\hline
table $:=$ $v : \text{value}$ $p : \text{(vb\_suffix | nnp)}$ $t : \text{table}$ & ``Mexican cuisine restaurants'' & ``Nobel prize award person''\\
\hline
table $:=$ $t : \text{table}$ ``with'' $v : \text{value}$ $p : \text{(vb\_suffix | nnp)}$ & ``restaurants with Mexican cuisine'' & ``hotels with Florida state''\\
\hline
table $:=$ $v : \text{value}$ $p : \text{jj\_suffix}$ $p : \text{(jj | jj\_prefix)}$ $t : \text{table}$ & ``5 star rated restaurants'' & ``Nobel prize award received person''\\
\bottomrule
\end{tabular}
\label{table:domain-specific-template}
\end{table*}
\fi


\iffalse
When generating complex queries, Genie depends on \textit{generic} templates to form the sketch of the query and \textit{domain-specific} templates to refer to the details. We introduce the two kinds of templates in following sections. %, and term them as domain-independent and domain-specific templates, respectively.
\fi

% The template
% \begin{tabbing}
% 1234\=\kill
% \>command $:=$ ``who'' $p : \text{vb}$ $v : \text{constant} \Rightarrow \text{Person}, p = v$
% \end{tabbing}

%\noindent produces commands of the form ``who works at Google''.  That's not the "form"!
% \noindent produces XXX, YYY, ZZZ when given \NLSchema XXX, YYY, ZZZ \TODO{Show 3 annotation examples}.
\iffalse
It does so by expanding the \textit{vb}
non-terminal with the VB canonical form of the ``worksFor'' property, and binding the property name to the variable
$p$. Similarly, it generates the constants ``Google'' and binds it to the $v$ variable. The semantic function combines
table, property and value to produce the desired query.
\fi

\iffalse
\subsection{Training data generation with Genie}
Genie generates semantic parsers for arbitrary programming language based on the definition of the
target language, a library of primitives (functions, tables, fields, etc.) in the language,
and developer-provided \textit{template} that map natural language to the operators in the language.

\webqa uses Genie by combining a built-in, generic set of templates, with developer-provided
and automatically-generated domain-specific templates. The domain-independent templates represent how different
part-of-speech, with associated \webtalk representation, are combined to form sentences and \webtalk queries.
The domain-specific templates provide additional query form for specific usages of tables and properties.
\fi

%\subsection{Generic templates}

\iffalse
\TODO{We need to describe in general what domain-independent templates are. And not just an example! They are handwritten?  How many of them?}


\TODO{IS the rest about domain-specific? I'm confused.}
The template generates sentences such as ``recipes that take less than 20 minutes to prepare''. It does so by combining the table expression
``recipes'', the prefix ``take'' and suffix ``to prepare'' of the VB form of the ``prepTime'' property, and the value ``20 minutes''.
The table is bound to the meta-variable $t$, the parameter to the meta-variable $p$, and the value to $v$. Those meta-variables are replaced
in the generated code, resulting in the \webtalk query ``Recipe, $\textit{prepTime} \le 20\text{min}$''.
\fi

\iffalse
\subsection{Domain-Specific Templates}
We wish to augment generic templates with domain-specific ones so the generated training data can include terminology specific to each domain.  To scale across all domains, we have developed a data-driven generator for domain-specific templates. 

For English queries, we have identified 8 common templates for specifying filters on tables, as shown in column 1 in Table~\ref{table:domain-specific-template}.  Columns 2 and 3 illustrate that which template gets used is highly dependent on the specific property.  We exhaustively apply each of the templates to every property in the \NLSchema by substituting the parameters with canonical forms of the right POS, and by replacing values with sampled data from the websites.  We test if the resulting phrases are used in practice by counting the number of exact matches returned by a web search engine.  We normalize the count to adjust for the fact that
longer queries have fewer exact matches. The 4 most commonly used templates are adopted for each property. 
\fi

\iffalse
 
are not sufficient to generate all possible natural questions, especially some special uses of phrases in each domain.
For this reason, \webqa uses a data-driven method to generate domain-specific templates for filters automatically.
Concretely, domain-specific templates describe how each property is commonly referred to in natural language together with the table name and value, and how that maps to a filter operation on the table.

Our method is based on a fixed list of template candidates. 
As shown in the first column of , these candidates are quite general among all possible domains. 

When employed with certain domain and one of its field, each candidate is expanded with the table name, canonical form of the property, and small sample of the values from the website data, forming the example queries as in Table~\ref{table:domain-specific-template}.
\webqa then employs a data-driven method: uses a web search API (such as \textit{Bing.com}) to determine which queries are more commonly used to refer to that property, based on the number of exact matches. 
We also take query length into consideration, as longer queries have fewer exact matches,
so we multiply the number of search results by an exponential factor that depends on the query length.
Finally, we rank all the template candidates according to the computed popularity and choose the top 4 as the domain-specific
templates for that property (listed as positive examples in Table~\ref{table:domain-specific-template}).
We exhaustively generates templates for each field in each domain, thus automatically generating domain-specific templates which refer to the \textit{filter} operation for that filed.

There are three domains in the examples of Table~\ref{table:domain-specific-template}: restaurants, hotels, and person. And example fields are servesCuisine, rating, and worksFor.
\fi
\iffalse
In the example of Table~\ref{}
Specifically, given the table's name (e.g. recipes), property's canonical form (e.g. ingredient), and several randomly sampled values 
of the property (e.g. chicken) from the target website, the patterns we have employed as candidates primitives are shown in Table~\ref{table:domain-specific-template}.


\TODO{JUST TALK ABOUT THE AUTOMATIC WITHOUT REFERRING TO THE MANUAL EFFORT.  IT IS CONFUSING.}

The main challenge in QA is understanding how data \TODO{What data} is referred to, and how that maps to a \textit{filter} operation on the table.
So developer's manual effort is to describe how to do filtering on certain property with natural language utterance.
For example, when filtering on the \texttt{recipeIngredient} property of recipe, the developer can provide ``\$x \{recipes\}'' 
and ``\{recipes with\} \$x ingredient'', where \$x is a placeholder which can be replaced by the name of the ingredient,
and ``\{recipes\}'' can be recursively expanded to a phrase that refers to recipes.
In \webqa, we aim to reduce developer's manual efforts by automating the generation of this form of templates.
\fi


==> sections/discussion.tex <==
%!TEX root = ../paper.tex
\subsection{Discussion}

Whether this approach applies to other natural languages is outside the scope of this paper.  However, our experience in drafting up templates for Chinese and Italian suggests that this is applicable to other languages as well. 
While the specific grammars are different, the concepts are similar across the languages. \TODO{how about sizes?}


==> sections/domain-variety.tex <==
%!TEX root = ../paper.tex
\subsection{Variety in Domain-Specific Ontology}
When referring to a database field in natural language, there are a variety of ways to describe it.
The variety does not limit to just synonyms, but also include different parts of speech (POS).
For example, Table~\ref{table:cuisine} shows different ways to search for restaurants by cuisine.

One can observe that, the same piece information in the database, 
have totally different phrases and POS in different queries.  
This shows that the existing template-based approach where each field has 
a single canonical form cannot capture the natural language variety in domain knowledge.

To address this problem, we propose to annotate each field with 
natural language phrases along with the corresponding part-of-speech information.
Then we apply manually-crafted generic templates to assemble natural language questions
based on the part-of-speech information.

In total, we identified seven POS categories that cover most of the ways fields are queried, 
as shown in Table~\ref{table:pos}.
Note that these POS are categorized based on how they can be used in natural language synthesis instead of parsing. 
For example, noun phrases are split into three categories to reflect the different use of properties:
noun phrase for property describes what the subject has, and can be used in constructs such as
``what/who has ...''; noun phrase for identity describes what the subject is, and can be used in constructs
such as ``what/who is ...''; noun phrase for implicit identity applies when the value of the field alone
is unambiguous enough to identify the subject, so it can be used in constructs where the subject is not specified.




\iffalse
\begin{table}
\caption{Different ways to search for Italian restaurants}
\small
\begin{tabular}{l|c|c}
\toprule
{\bf Query} & {\bf Phrase} & {\bf POS}\\
\midrule
show me restaurants with Italian cuisine? & Italian cuisine & noun\\
\hline
what restaurants offer Italian food? & offer Italian food & verb\\
\hline
show me Italian restaurants & Italian & adjective \\
\bottomrule
\end{tabular}
\label{table:cuisine}
\end{table}

\paragraph{Base noun phrase}
The base noun phrase of a parameter is used for describing the parameter without context. 
In particular, it is supposed to be used without a value round it. This includes projection questions, count of a property.
For example, ``servesCuisine'' property has a base noun phrase``cuisine'', 
and can be used to generate sentences like ``what is the cuisine of this restaurant?''.

\paragraph{Noun phrase for property}
A property field is a field representing what the subject has. 
For examples, ``alumniOf'' has a noun phrase for property ``degree from \#'',
where \# indicates where the value should be placed. 
This annotation can be used to generate sentences like ``who has a degree from X university?''.

\paragraph{Noun phrase for identity}
An identity field is a field representing what the subject is.
For example, ``alumniOf'' has a noun phrase for identity ``alumni of \#''
This annotation can be used to generate sentences like ``who are alumni of X university?''

\paragraph{Noun phrase for implicit identity}
An implicit identity field is a field that the value of the field alone is unambiguous to identify the subject.
So when constructing the natural language query, we don't need to explicitly mention the name of the subject.
For example, ``category'' property can be used as an implicit identity for product domain. So we can say ``search for tablets'' without mentioning products in the sentences. 

\paragraph{Verb phrase}
Lots of properties can also be used in verb phrase.
For example, ``servesCuisine'' can be referred as ``serves \# food''.
We can synthesize ``which restaurant serves Italian food?'' based on this annotation.

\paragraph{Passive verb phrase}
Passive verb phrase is another common POS in natural language questions.
For example, ``worksFor'' property can be referred in passive verb phrase ``employed by'', and we can construct questions such as ``who is employed by X company?'' and ``show me people employed by X company''. 

\paragraph{Adjective phrase}
Some of the property values can also be used as an adjective of the subject.
``servesCuisine'' property is one of the examples. 
We can say ``show me Italian restaurants'' where we simply put the value in front of
restaurants without mentioning the property.  

\paragraph{Preposition phrase}
Preposition phrase is used similarly as passive verb phrased.
For example ``worksFor'' property has preposition phrase ``from'', and we can generate
questions like ``who is from X company'' or ``show me people from X company''.
\fi

We use information from external knowledge bases to bootstrap the natural language annotations when available.
For example, Wikidata.org contains equivalent schema.org properties, and each property has 
a list of natural language labels to describe how they are used in natural language. 
We apply a rule-based heuristic algorithm based on standard POS tagger to decide which category each label belongs to.
Domain experts can correct the mistakes made by the heuristics and supply additional annotations to improve the coverage.


==> sections/overview.tex <==
%!TEX root = ../paper.tex
\section{System Overview}
\label{sec:overview}



%Our taxonomy of questions can be applied to the general synthesis methodology to generate a dataset and train a neural semantic parser~\cite{overnight, geniepldi19}.
%The result is a complete pipeline that automatically generates a semantic parser that can handle questions in each domain.
%Furthermore, domain experts the ability to improve the accuracy of the system.


\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{./figures/diagram.pdf}
\caption[]{Schema2QA pipeline.}
\label{fig:overview}
\Description{}
\end{figure}


%To do so, we introduce an executable formal language called DBTalk, and the \webqa toolkit to train a semantic parser to translate natural language questions into the corresponding DBTalk queries.

\webqa is a tool that creates \QandA agents from database schemas.  To answer questions on the structured web, we apply this tool on the Schema.org schema.  
Fig.~\ref{fig:overview} shows the high-level system architecture.  The first module, NLSchema Builder, turns the graph-based Schema.org into a relational database augmented with a small amount of manual natural-language annotation per property in the schema.  

The second module, Data Synthesizer, generates training data for the semantic parser that translates natural language into \DBTalk. Built into the Data Synthesizer is a comprehensive set of {\em generic query templates}. The synthesizer applies these templates to the property annotations in the input schema to create a large set of training data. 
Then both the synthetic and paraphrased sets are augmented by replacing parameters with 
the actual values in the knowledge base. 
This allows us to expose more real values to the neural network
to learn how they match to different properties.
 
The augmented dataset is then used to train our third module, a novel BERT-LSTM neural semantic parser. 
At inference time, questions are translated by the parser to generate the \DBTalk, which can be executed to retrieve the answer. 

\webqa is designed to support iterative refinement.  Developers can improve the result of the \QandA system by analyzing the errors of the system and adding more annotations to the database properties, or adding to the generic query templates.   

\iffalse
Because \webqa produces a training set and a trained model for each skill, instead of
reusing an existing model, website owners can customize the skills. 
They can collect the validation set to identify weaknesses in the synthesized data, and augment the data with additional natural language annotations.
They can also add useful queries and high-level concepts manually, for the questions that they care about,
in the form of templates. These templates can be site-specific, if they refer
to site-specific functionality, or they can be added to the general taxonomy of web questions to grow the
capabilities of all skills.
\fi



%and then retrieves the answer by executing the code directly.
%\webqa uses the canonical forms and types to display the results of the query.

%If the query returns many fields, a default priority is used to present the most important ones. For each table, developers can override the formatting information. 

\iffalse
Here we present a high-level overview of the \webqa system, as shown in 
The first step of the methodology takes the schema definitions from the database, as well as the domain-specific natural language information
(canonical forms and part-of-speech (POS) information of each property).
If \webqa is applied to schema.org, this entails building a \NLSchema knowledge base.
The knowledge base includes both the website data, and the natural language  of each property.
\webqa includes a tool to automatically transform the whole Schema.org representation into \NLSchema.  
Additional natural language information can be supplied manually to improve its quality. 

To represent complex questions, \webqa uses a new query language, called \webtalk.
\webtalk is an executable formal language inspired by SQL, 
but is designed to capture the intent of the user succinctly,
and be easy to synthesize. 
\webqa then uses a template-based algorithm to synthesize a large set of training examples for each domain.
% The templates combine canonical annotations tagged with part-of-speech from each domain into natural sentences and their corresponding DBTalk code.
% A small sample of synthesized examples are then paraphrased by crowd-workers. 
Finally, \webqa trains a neural semantic parser to translate natural language into \webtalk code,
\fi

% Both synthetic data and paraphrase data are used to train a semantic parser using a noval BERT-LSTM model. 
% In our experiments, we find the accuracy of our model outperforms the state-of-the-art models consistently.

%Developers are expected to use the validation set to identify weaknesses in the synthesized data, and augment the data with additional natural language annotations.
%Once the parser is trained, we can use it to answer questions for any websites in that domain that use Schema.org. 

\iffalse
The custom QA systems generated by \webqa can answer complex questions
with high accuracy thanks to design of \DBTalk and the large diverse training data
it synthesizes.
Table~\ref{table:comparison} shows a sample of questions that can be answered 
by skills generated by Schema2QA. 
In contrast, today’s commercial assistants cannot answer most of such questions.
\fi


==> sections/question-modeling.tex <==
%!TEX root = ../paper.tex
\section{Modeling of Database Questions}

==> sections/representation-compressed.tex <==
%!TEX root = ../paper.tex
\section{\NLSchema Knowledge Base}
\label{sec:representation}
%We have developed a set of heuristics that leverages schema.org data in websites to translate schema.org into NL-Schema. 

Schema.org is a markup vocabulary created to help
search engines understand and index structured data across the web. 
Here, we introduce Schema.org and describe how we extend it to natural language queries. 

\subsection{Data model of Schema.org}
% do not change this back, nodes are not classes, nodes *belong to* classes
Schema.org is based on RDF, and uses a graph data model, where nodes represent objects. Nodes are connected by \textit{properties}
and are grouped in \textit{classes}.
Classes are arranged in a multiple inheritance hierarchy where each class can be a subclass of 
multiple other classes, and the ``Thing'' class is the superclass of all classes.
There is also a parallel hierarchy where the literal data types are defined.
By convention, all class names start with an uppercase letter, while property names start with a lowercase letter.

%domain is just the regular maths domain, not a defined term
Each property's domain consists of one or more classes that can possess that property.
 The same property can be used in separate domains. For example, ``Person'' and ``Organization'' classes both use the ``owns'' property. Subclasses of a class in the domain of a certain property can also make use of that property.

Each property's range consists of one or more classes or primitive types.  
Additionally, as having any data is considered better than none, the ``Text'' type (free text) is always implicitly included in a property's range.  For properties where free text is the recommended or only type expected, e.g. the ``name'' property, ``Text'' is explicitly declared as the property type. 

\iffalse
Schema.org is organized in layers, with a ``core'' layer representing the portion agreed by
all users, a ``pending'' layer including proposed addition to the core, and various
extension layers (e.g., ``bib'', ``auto''). Here we only consider 
the core layer.
\fi

\subsection{NL-Schema Representation}
We propose a new data model \NLSchema to store website data.
\NLSchema provides the domain-specific information used in the synthesis of training data.
To facilitate the generation, \NLSchema uses a relational data model, where each table contains a fixed set of properties with fixed types. An example is shown in Fig.~\ref{fig:example-schema}. \webqa includes a converter tool
that leverages the Schema.org definitions and the data in websites to translate the graph-based Schema.org representation automatically into \NLSchema. 

\begin{figure}[h]
\begin{lstlisting}
skill Restaurant {
  Thing(
    name: String #_[prop=["name"]],
    image: Picture #_[prop=["image", "picture"]],
    description: String #_[prop=["description"]], ...
  );
  Place extends Thing(
    aggregateRating: {                      
      reviewCount: Number #_[prop=["review count"]],
      ratingValue: Number #_[
        prop=["rating"],
        passive_verb=["rated # star"}] 
      ]
    }, ... 
  );
  Organization extends Thing();
  LocalBusiness extends Place, Organization();
  FoodEstablishment extends LocalBusiness(
    servesCuisine: String #_[ 
      prop=["cuisine", "food type"], 
      verb=["serves # cuisine", "offer # food"] 
    ], ...
  );
  Restaurant extends FoodEstablishment();
}

\end{lstlisting}
\caption{\NLSchema representation for Restaurant}
\label{fig:example-schema}
\end{figure}

\iffalse
\begin{figure}
\small
\begin{tabbing}
123\=12345678901234567890123\=\kill\\
\>Skill $s$ \>$\texttt{skill}~~\texttt{\{}~~\textit{tdef}^+~~\texttt{\}}$\\
\>Table Definition $\textit{tdef}$ \>$\textit{tn}~\left[\texttt{extends}~~\textit{tn}^+\right]^?~\texttt{(}~\textit{fdef}^*~\texttt{)}$\\
\>Field Definition $\textit{fdef}$ \>$\textit{fn}~~:~~\textit{type}~~\texttt{\#\_[}~~\textit{ann}^*~~\texttt{]}$\\
\>Annotation $\textit{ann}$ \>$\textit{pos}=\textit{cf}~~\vert~~\texttt{nnv}=\texttt{true}~~\vert~~\texttt{jjv}=\texttt{true}$\\
\>Canonical Form $\textit{cf}$ \>$\text{literal}~~\vert~~\texttt{\{}~\texttt{prefix}=\text{literal}~,~\texttt{suffix}=\text{literal}~\texttt{\}}$\\
\>Part-of-Speech $\textit{pos}$ \>$\texttt{nnp}~~\vert~~\texttt{nni}~~\vert~~\texttt{vb}~~\vert~~\texttt{jj}$\\
\>Type $\textit{type}$ \>$\texttt{Entity}(\textit{tn})~~\vert~~\texttt{String}~~\vert~~\texttt{Number}~~\vert~~\texttt{Time}~~\ldots$\\
\>Table name $\textit{tn}$\>identifier\\
\>Field name $\textit{fn}$\>identifier
\end{tabbing}
\caption{The formal definition of \NLSchema.}
\label{fig:NL-Schema}
\end{figure}
\fi

\paragraph{Tables and record types.}
In \NLSchema, we distinguish between {\em entity} and {\em non-entity} classes. 
Entity classes are those that refer to well-known meaningful identities, such as people, organization, places, events, URLs, with names that the user can recognize.  All other classes are considered non-entity. They can only be referred to as properties of other classes. %Note the converse is not true: a property can refer to an entity class. 
This distinguish between entity and non-entity classes matches
how each class is used in natural language, and simplifies the query representation. 

An entity class is represented as a table, whose properties make up the columns.  
The column may be of a primitive type, a reference to another entity class, or a record type.
Non-entity classes are represented as anonymous record types, with the exception of recursive classes.   
\DBTalk does not have recursive record types, where a record type has a field with the same type.  
Recursive non-entity classes are mapped to nameless tables, instead of record types. 
%\TODO{Can't follow: simply you are saying a review can be reviewed?
% TODO ANSWER: yes
For example, the ``Review'' class is a non-entity class, because it inherits the ``review'' property from ``CreativeWork'', and that property also refers to the ``Review'' class.
In practice, most classes only use a subset of their properties.
We use data scraped from websites to eliminate the properties that are not used. This limits the vocabulary to only the relevant terms.



%When mapping schema.org to \NLSchema, \webqa makes use of the website data.  -- this is not the point of the paragraph, don't lead with it. 

\iffalse
When a class is used as a property, it often uses only a subset of all the possible fields. Consider the non-entity class ``Rating''. % When referred as the ``contentRating'' property of the ``Movie'' class, it uses field \TODO{XXX}; 
When referred as the ``aggregateRating'' property of the ``Restaurant'' class, it uses fields ``reviewCount'' and ``ratingValue'';
when referred as the ``reviewRating'' property of the ``Review'' class, it uses fields ``ratingValue'' and might use the ``author'' field.
We use Schema.org data scraped from websites to determine the fields used in practice for each class's property, and create a custom record type holding only such fields for that property. This limits the vocabulary to only the relevant terms for each class's property. 
\fi

\paragraph{Identifying property types.}
Template-based synthesis relies on precise type information to generate meaningful questions. When mapping from Schema.org in particular, this requires identifying the cardinality of the property, to distinguish scalar and array properties. For example, for plural properties such as ``review'' we can ask ``how many reviews does a restaurant have?'',
and ``what restaurant has the most reviews?''. 
\webqa uses a number of heuristics to identify arrays, based on the Schema.org property name, type, and description. Empirically, we found our heuristics works well in the 3 domains we evaluated, with the exception of properties of the ``Thing'' class such as ``image'' and ``description'', which are described as plural in the comment, but have one value per object in practice.

Many properties use a union type in Schema.org. To avoid ambiguity when parsing natural language, this is not supported in \NLSchema.  For each property, \webqa picks among the types in its range the one with the highest priority, which is defined in decreasing order: record types, primitive types, entity references, and finally strings.  All website data is then cast to the chosen type.

\iffalse
Since correctly distinguishing singular and plural properties is necessary to generate good
training sentences, we introduce cardinality to NL-Schema fields.  For example, for plural properties such as ``review'' we can ask ``how many reviews does a restaurant have?'',
and ``what restaurant has the most reviews?''. 
\fi

\iffalse
\webqa considers any Schema.org property with ``ItemList'' type as an array. It also heuristically analyzes the documentation comment provided on Schema.org to identify arrays. Furthermore, when the element type of the array is not provided by Schema.org, \webqa heuristically infers it from the property name.
Empirically, we found our heuristics works well in the 3 domains we evaluated, with the exception of properties
of the ``Thing'' class such as ``image'' and ``description'', which are described as plural in the comment, but have one value per object in practice.
\fi
%\webqa also needs to infer the element type of each array property, when this information is not provided in 
%If the property has type ``ItemList'' or a subclass of ``ItemList'', and no other types in its range, \webqa heuristically infers the correct
%element type based on the property name.

\iffalse
{\bf Union types.}
%\TODO{How can you "heuristically choose one type"?  This is really ad hoc.  How do you normalize data types? They don't match, they don't match.  How do you get to "prefer" structure types, and falls back to whatever.  This is not scientific.}
For compatibility with existing websites and extensibility, the range of many properties in Schema.org includes multiple classes, effectively creating a union type.  To avoid ambiguity when parsing natural language, and to
avoid having to resolve the type dynamically at runtime, which can lead to missing data and confusion, 
\NLSchema does not support union types.  For each property, it picks among the types in its range the one with the highest priority, which is defined in decreasing order: record types, \webtalk primitive types, entity references, and finally strings.  All website data is cast to the chosen type as follows: 
%\TODO{The casting operator is incomplete here:}
If the data contains a primitive value or a record where an entity reference is expected, \webqa creates new entities, and assigns new unique IDs. Conversely, if the
data contains a record where a primitive value or an entity reference is expected, \webqa reports a warning and selects a property of that record
as the primitive value. Note that website data often do not respect the type declared in Schema.org; in that case, \webqa will automatically cast the data to the correct type or discard the value.
%TODO{According to your algorithm if there is a record type, the record type will be picked.  You don't ever have to cast down, but just up.  Please clean this up thoroughly please.}
\fi

\paragraph{Automatic canonical forms.}
When converting to \NLSchema, \webqa automatically generates a canonical form for each property, based on the property name
and type. Camel-cased names are converted into multiple words; redundant words at the beginning and end are removed. \webqa uses a POS tagger and heuristics to identify the POS of the generated canonical form. More details of all POS categories supported by \NLSchema and 
how they helped us synthesize natural sentences is describe in 
Section~\ref{sec:algorithm}. 


\paragraph{Displaying results.}
\webqa uses the canonical forms and types to display the results of the query. If the query returns many fields, a default priority is used to present the most important ones. For each table, developers can override the formatting information. 

\iffalse
For example, it converts ``worksFor'' to ``works for'', and ``ratingValue'' to ``rating''. 
\webqa removes the table name or the names of the parent record type from the property name, if present.  
For example, ``reviewRating'' is converted to ``rating''. 
\webqa also recognizes the verbs ``has'' and ``is'', which are commonly used as prefixes of property names in Schema.org,
and uses to identify the correct part of speech for the generated canonical form. Developers can manually add more canonical forms or refine the generated ones.
\fi

\iffalse
Alternatively, webqa provides a default representation, based on the canonical forms and types of the parameters.
In the default representation, parameters are ranked by heuristic importance based on name and type,
and only the most important parameters are preserved. In either case, the representation is 
automatically adapted by \webqa to match the fields the user is interested in, and to discard missing
or invalid data.
\fi



%It does so by annotating each property with a list of : short phrases
% that refer to the property. 

\iffalse
\TODO{Bad English: "each property" of what? None of the sentences follow from each other.  
Just describe the design.
Just forget what the schema.org has or not has.  Just describe the design and its rationale.  
}
To be able to generate meaningful natural language sentences using each property, we need each property
to be annotated with how it is commonly used. At the same time, because it is not designed for QA, schema.org
does not have any natural language annotation.
% To overcome this disadvantage of schema.org, we introduces natural language annotation for fields.

\TODO{This is too cryptic.  What is canonical form?  What is it used for?}
In \webqa, developers CAN? define exactly how the property will be referred to in natural language,
specifying both one or more \text{canonical forms}, and their corresponding \textit{part-of-speech}.
\TODO{NO CLUE WHAT THIS IS ... NO EXAMPLE}
For each canonical form, the developer can specify both a part should precede the property value (``prefix'')
and a part that should follow the property value (``suffix'').
\TODO{WHAT DO YOU MEAN ALTERNATIVELY?  YOU TOLD ME THAT EVERYTHING IS AUTOMATIC}
Alternatively, \webqa can automatically generate annotations for each property, based on the property name
and type. It first converts the camel-cased names into multiple words and removes redundant words at the end such 
as ``value'' and ``content''. \TODO{WHY ARE VALUE, CONTENT REDUNDANT}

It also recognize commonly used verbs, ``has'' and ``is'', and checks the part-of-speech tags to decide
the grammar category to use.  \TODO{WHERE DO YOU GET THESE TAGS?}


\iffalse
Schema.org is designed primarily to provide a vocabulary of structured data to help search engines to better understand the web.
There is a gap between natural language and the schemas.
In particular, due to the lack of name space, all property names are used globally.
As a result, property names are over specified for a given context or domain, and differ from how people refer to them in natural language.
For example, to distinguish the ratings from customers and the star rating for hotels and restaurants, the twp properties are named \texttt{aggregateRating} and \texttt{starRating}. While in reality these two term will almost never appear in the related queries. 
\fi

\TODO{Explain how these annotation types are used.  I don't understand your acronyms at all.  What is JJ? NNP? Where do these names come from}

In particular, we propose 6 different annotation types based on the grammar category of the field name and its value: \TODO{I don't understand the English of these paragraphs.}

\TODO{Now describe the comparison.}


\iffalse
For English, we propose a data-driven algorithm to automatically generate such  natural language annotation based on the field name and real-world data.
The approach can potentially be applied to other languages with the help of machine translation. 
Developers can also manually annotate based on the domain knowledge and the particular use case and data. Note that each field can use one one or more annotation types, and each annotation takes an array of strings, so developers can provide all different ways the field might be used in real life.
\fi 
\fi


==> sections/representation.tex <==
%!TEX root = ../paper.tex
\section{Adapting schema.org for NLP}
\label{sec:representation}
%We have developed a set of heuristics that leverages schema.org data in websites to translate schema.org into NL-Schema. 

Schema.org is a markup vocabulary created to help
search engines understand and index structured data across the web. Here, we introduce Schema.org and describe how we extend it to natural language queries. 

\subsection{Data model of Schema.org}
% do not change this back, nodes are not classes, nodes *belong to* classes
Schema.org is based on RDF, and uses a graph data model, where nodes represent objects. Nodes are connected by \textit{properties}
and are grouped in \textit{classes}.
Classes are arranged in a multiple inheritance hierarchy where each class can be a subclass of 
multiple other classes, and the ``Thing'' class is the superclass of all classes.
There is also a parallel hierarchy where the literal data types are defined.
By convention, all class names start with an uppercase letter, while property names start with a lowercase letter.

%domain is just the regular maths domain, not a defined term
Each property's domain consists of one or more classes that can possess that property.
 The same property can be used in separate domains; e.g., ``Person'' and ``Organization'' classes both use the ``owns'' property. Subclasses of a class in the domain of a certain property can also make use of that property.

Each property's range consists of one or more classes or primitive types.  
Additionally, as having any data is considered better than none, the ``Text'' type (free text) is always implicitly included in a property's range.  For properties where free text is the recommended or only type expected, e.g. the ``name'' property, ``Text'' is explicitly declared as the property type. 

Schema.org is organized in layers, with a ``core'' layer representing the portion agreed by
all users, a ``pending'' layer including proposed addition to the core, and various
extension layers (e.g., ``bib'', ``auto''). Here we only consider 
the core layer.

\subsection{NL-Schema Representation}
\NLSchema, and templates derived from it, provide the domain-specific information used in the grammar-driven generation of training data.
To facilitate the generation, \NLSchema uses a relational data model, where each table contains a fixed set of properties with fixed types.  The grammar is shown in Fig.~\ref{fig:NL-Schema}, and an example is shown in Fig.~\ref{fig:example-schema}. \webqa includes a converter tool
that leverages the Schema.org definitions and the Schema.org data in websites to translate the graph-based Schema.org representation automatically into \NLSchema. 

\begin{figure}
\small
\begin{tabbing}
123\=12345678901234567890123\=\kill\\
\>Skill $s$ \>$\texttt{skill}~~\texttt{\{}~~\textit{tdef}^+~~\texttt{\}}$\\
\>Table Definition $\textit{tdef}$ \>$\textit{tn}~\left[\texttt{extends}~~\textit{tn}^+\right]^?~\texttt{(}~\textit{fdef}^*~\texttt{)}$\\
\>Field Definition $\textit{fdef}$ \>$\textit{fn}~~:~~\textit{type}~~\texttt{\#\_[}~~\textit{ann}^*~~\texttt{]}$\\
\>Annotation $\textit{ann}$ \>$\textit{pos}=\textit{cf}~~\vert~~\texttt{nnv}=\texttt{true}~~\vert~~\texttt{jjv}=\texttt{true}$\\
\>Canonical Form $\textit{cf}$ \>$\text{literal}~~\vert~~\texttt{\{}~\texttt{prefix}=\text{literal}~,~\texttt{suffix}=\text{literal}~\texttt{\}}$\\
\>Part-of-Speech $\textit{pos}$ \>$\texttt{nnp}~~\vert~~\texttt{nni}~~\vert~~\texttt{vb}~~\vert~~\texttt{jj}$\\
\>Type $\textit{type}$ \>$\texttt{Entity}(\textit{tn})~~\vert~~\texttt{String}~~\vert~~\texttt{Number}~~\vert~~\texttt{Time}~~\ldots$\\
\>Table name $\textit{tn}$\>identifier\\
\>Field name $\textit{fn}$\>identifier
\end{tabbing}
\caption{The formal definition of \NLSchema.}
\label{fig:NL-Schema}
\end{figure}


{\bf Tables and record types.}
In \NLSchema, we distinguish between {\em entity} and {\em non-entity} classes. 
Entity classes are those that refer to well-known meaningful identities, such as people, organization, places, events, URLs, with names that the user can recognize.  All other classes are considered non-entity; they can only be referred to as properties of other classes. %Note the converse is not true: a property can refer to an entity class. 

An entity class is represented as a table, whose properties make up the columns.  
The column may be of a primitive type, a reference to another entity class, or a record type.
Non-entity classes are represented as anonymous record types, with the exception of recursive classes.   
\DBTalk does not have recursive record types, where a record type has a field with the same type.  
Recursive non-entity classes are mapped to nameless tables, instead of record types. 
%\TODO{Can't follow: simply you are saying a review can be reviewed?
% TODO ANSWER: yes
For example, the ``Review'' class is a non-entity class, because it inherits the ``review'' property from ``CreativeWork'', and that property also refers to the ``Review'' class.

%When mapping schema.org to \NLSchema, \webqa makes use of the website data.  -- this is not the point of the paragraph, don't lead with it. 

When a class is used as a property, it often uses only a subset of all the possible fields. Consider the non-entity class ``Rating''. % When referred as the ``contentRating'' property of the ``Movie'' class, it uses field \TODO{XXX}; 
When referred as the ``aggregateRating'' property of the ``Restaurant'' class, it uses fields ``reviewCount'' and ``ratingValue'';
when referred as the ``reviewRating'' property of the ``Review'' class, it uses fields ``ratingValue'' and might use the ``author'' field.
We use Schema.org data scraped from websites to determine the fields used in practice for each class's property, and create a custom record type holding only such fields for that property. This limits the vocabulary to only the relevant terms for each class's property. 

{\bf Array types.}
Since correctly distinguishing singular and plural properties is necessary to generate good
training sentences, we introduce cardinality to NL-Schema fields.  For example, for plural properties such as ``review'' we can ask ``how many reviews does a restaurant have?'',
and ``what restaurant has the most reviews?''. 

\webqa considers any Schema.org property with ``ItemList'' type as an array. It also heuristically analyzes the documentation comment provided on Schema.org to identify arrays. Furthermore, when the element type of the array is not provided by Schema.org, \webqa heuristically infers it from the property name.
Empirically, we found our heuristics works well in the 3 domains we evaluated, with the exception of properties
of the ``Thing'' class such as ``image'' and ``description'', which are described as plural in the comment, but have one value per object in practice.
%\webqa also needs to infer the element type of each array property, when this information is not provided in 
%If the property has type ``ItemList'' or a subclass of ``ItemList'', and no other types in its range, \webqa heuristically infers the correct
%element type based on the property name.

{\bf Union types.}
%\TODO{How can you "heuristically choose one type"?  This is really ad hoc.  How do you normalize data types? They don't match, they don't match.  How do you get to "prefer" structure types, and falls back to whatever.  This is not scientific.}
For compatibility with existing websites and extensibility, the range of many properties in Schema.org includes multiple classes, effectively creating a union type.  To avoid ambiguity when parsing natural language, and to
avoid having to resolve the type dynamically at runtime, which can lead to missing data and confusion, 
\NLSchema does not support union types.  For each property, it picks among the types in its range the one with the highest priority, which is defined in decreasing order: record types, \webtalk primitive types, entity references, and finally strings.  All website data is cast to the chosen type as follows: 
%\TODO{The casting operator is incomplete here:}
If the data contains a primitive value or a record where an entity reference is expected, \webqa creates new entities, and assigns new unique IDs. Conversely, if the
data contains a record where a primitive value or an entity reference is expected, \webqa reports a warning and selects a property of that record
as the primitive value. Note that website data often do not respect the type declared in Schema.org; in that case, \webqa will automatically cast the data to the correct type or discard the value.
%TODO{According to your algorithm if there is a record type, the record type will be picked.  You don't ever have to cast down, but just up.  Please clean this up thoroughly please.}

{\bf Part-of-Speech Annotations.}
When converting to \NLSchema, \webqa automatically generates a canonical form for each property, based on the property name
and type. It converts the camel-cased names into multiple words and removes redundant words at the end of property names.   
For example, it converts ``worksFor'' to ``works for'', and ``ratingValue'' to ``rating''. 
\webqa removes the table name or the names of the parent record type from the property name, if present.  
For example, ``reviewRating'' is converted to ``rating''. 
\webqa also recognizes the verbs ``has'' and ``is'', which are commonly used as prefixes of property names in Schema.org,
and uses to identify the correct part of speech for the generated canonical form. Developers can manually add more canonical forms or refine the generated ones.
The canonical forms and types are also used in the displaying the results of the query. If the query returns many fields, a default priority is used to present the most important ones. For each table, domain experts can override the formatting information. 

\iffalse
Alternatively, webqa provides a default representation, based on the canonical forms and types of the parameters.
In the default representation, parameters are ranked by heuristic importance based on name and type,
and only the most important parameters are preserved. In either case, the representation is 
automatically adapted by \webqa to match the fields the user is interested in, and to discard missing
or invalid data.
\fi



%It does so by annotating each property with a list of : short phrases
% that refer to the property. 

\iffalse
\TODO{Bad English: "each property" of what? None of the sentences follow from each other.  
Just describe the design.
Just forget what the schema.org has or not has.  Just describe the design and its rationale.  
}
To be able to generate meaningful natural language sentences using each property, we need each property
to be annotated with how it is commonly used. At the same time, because it is not designed for QA, schema.org
does not have any natural language annotation.
% To overcome this disadvantage of schema.org, we introduces natural language annotation for fields.

\TODO{This is too cryptic.  What is canonical form?  What is it used for?}
In \webqa, developers CAN? define exactly how the property will be referred to in natural language,
specifying both one or more \text{canonical forms}, and their corresponding \textit{part-of-speech}.
\TODO{NO CLUE WHAT THIS IS ... NO EXAMPLE}
For each canonical form, the developer can specify both a part should precede the property value (``prefix'')
and a part that should follow the property value (``suffix'').
\TODO{WHAT DO YOU MEAN ALTERNATIVELY?  YOU TOLD ME THAT EVERYTHING IS AUTOMATIC}
Alternatively, \webqa can automatically generate annotations for each property, based on the property name
and type. It first converts the camel-cased names into multiple words and removes redundant words at the end such 
as ``value'' and ``content''. \TODO{WHY ARE VALUE, CONTENT REDUNDANT}

It also recognize commonly used verbs, ``has'' and ``is'', and checks the part-of-speech tags to decide
the grammar category to use.  \TODO{WHERE DO YOU GET THESE TAGS?}


\iffalse
Schema.org is designed primarily to provide a vocabulary of structured data to help search engines to better understand the web.
There is a gap between natural language and the schemas.
In particular, due to the lack of name space, all property names are used globally.
As a result, property names are over specified for a given context or domain, and differ from how people refer to them in natural language.
For example, to distinguish the ratings from customers and the star rating for hotels and restaurants, the twp properties are named \texttt{aggregateRating} and \texttt{starRating}. While in reality these two term will almost never appear in the related queries. 
\fi

\TODO{Explain how these annotation types are used.  I don't understand your acronyms at all.  What is JJ? NNP? Where do these names come from}

In particular, we propose 6 different annotation types based on the grammar category of the field name and its value: \TODO{I don't understand the English of these paragraphs.}

\TODO{Now describe the comparison.}


\iffalse
For English, we propose a data-driven algorithm to automatically generate such  natural language annotation based on the field name and real-world data.
The approach can potentially be applied to other languages with the help of machine translation. 
Developers can also manually annotate based on the domain knowledge and the particular use case and data. Note that each field can use one one or more annotation types, and each annotation takes an array of strings, so developers can provide all different ways the field might be used in real life.
\fi 
\fi


==> sections/variety2.tex <==
%!TEX root = ../paper.tex
\section{Natural Language to \DBTalk}
\label{sec:nl-to-dbtalk}

The principle behind neural semantic parsers is to let the neural network generalize from many possible sentences annotated with their meaning in a formal representation. However, because languages are compositional, the neural network must see many possible combinations in order not to overfit. In contrast, compositionality is baked into grammar-based parsers, but they fail to handle the irregularities and contextual variations in natural language.  We propose to use templates to generate perfectly annotated natural language sentences to provide coverage and to teach the neural network compositionality, and we use paraphrases to expose the network to more variety in natural language. Our approach allows the network to generalize and understand natural language with significantly less manually labeled data. 

\setlength\tabcolsep{3pt}
\begin{table*}[tb]
\caption{Canonical templates mapping natural language to \DBTalk code.}
\vspace{-0.5em}
\small
\centering
\begin{tabular}{p{1.4cm}|p{0.84cm}p{5.4cm}|p{3.7cm}|p{5.3cm}}
\toprule
{\bf Operator}               & \multicolumn{2}{c|}{\bf Natural language template}           & {\bf \DBTalk}                                       & \bf Minimal Example \\
\hline
\multirow{3}{*}{Selection}   & table $:=$& $t : \textit{table}$ with $f : \textit{fname}$ equal to $v : \textit{value}$     & $t, f = v$   & [restaurants] with [cuisine] equal to [Chinese] \\ 
                             & $\quad\quad\;\,\vert$& $t : \textit{table}$ with $f : \textit{fname}$ greater than $v : \textit{value}$ & $t, f \ge v$ & [restaurants] with [rating] greater than [3.5]  \\
                             & $\quad\quad\;\,\vert$& $t : \textit{table}$ with $f : \textit{fname}$ less than $v : \textit{value}$    & $t, f \le v$ & [restaurants] with [rating] less than [3.5]  \\
                             & $\quad\quad\;\,\vert$& $t : \textit{table}$ with $f : \textit{fname}$ containing $v : \textit{value}$   & $t, \text{contains}(f, v)$ & [people] with [employers] containing [Google]  \\
\hline
\multirow{2}{*}{Ranking}     & table $:=$& the $t : \textit{table}$ with the min $f : \textit{fname}$      & $(\texttt{sort}~f~\texttt{asc}~\texttt{of}~t)[1]$  & the [restaurants] with the min [rating] \\
                             & $\quad\quad\;\,\vert$& the $t : \textit{table}$ with the max $f : \textit{fname}$      & $(\texttt{sort}~f~\texttt{desc}~\texttt{of}~t)[1]$ & the [restaurants] with the max [rating] \\
                             & $\quad\quad\;\,\vert$& the $n : \textit{number}$ $t : \textit{table}$ with the min $f : \textit{fname}$  & $(\texttt{sort}~f~\texttt{asc}~\texttt{of}~t)[1:n]$ & the [3] [restaurants] with the min [rating] \\
                             & $\quad\quad\;\,\vert$& the $n : \textit{number}$ $t : \textit{table}$ with the max $f : \textit{fname}$  & $(\texttt{sort}~f~\texttt{desc}~\texttt{of}~t)[1:n]$ & the [3] [restaurants] with the max [rating] \\
\hline
\multirow{1}{*}{Join}        & table $:=$& the $t_1 : \textit{table}$ of $t_1 : \textit{table}$           & $(t_2~\texttt{join}~t_1), \text{in\_array}(id, t_2)$ & [reviews with ...] of [restaurants with ...]     \\
\hline
\multirow{1}{*}{Quantifiers} & table $:=$& $t_1 : \textit{table}$ with $t_2 : \textit{table}$             & $t_1, \texttt{exists}(t_2, \text{in\_array}(id, t_1))$ & [restaurants with ...] with [reviews with ...] \\
                             & $\quad\quad\;\,\vert$& $t_1 : \textit{table}$ with no $t_2 : \textit{table}$          & $t_1, !\texttt{exists}(t_2, \text{in\_array}(id, t_1))$ & [restaurants with ...] with [no reviews with ...] \\
\hline
Projection                   & fref $:=$& the $f : \textit{fname}$ of $t : \textit{table}$                    & $f~\texttt{of}~t$         & the [cuisine] of [restaurants] \\
\hline
\multirow{2}{*}{Aggregation} & fref $:=$& the number of \textit{table}                     & $\texttt{aggregate}~\text{count}~\texttt{of}~t$ & the number of [restaurants] \\
                             & $\quad\quad\;\,\vert$& the \textit{op} $f : \textit{fname}$ in $t : \textit{table}$               & $\texttt{aggregate}~\textit{op}~f~\texttt{of}~t$ & the [average] [rating] of [restaurants] \\
\hline
\multirow{2}{1.5cm}{Row-wise function} & fref $:=$& the distance of $t : \textit{table}$ from $l : \textit{loc}$        & $\texttt{compute}~\text{distance}(\textit{geo}, l)~\texttt{of}~t$ & the distance of [restaurants] from [here] \\
                             & $\quad\quad\;\,\vert$& the number of $f : \textit{fname}$ in $t : \textit{table}$          & $\texttt{compute}~\text{count}(f)~\texttt{of}~t$ & the number of [reviews] in [restaurants] \\
\bottomrule
\end{tabular}
\label{table:db-ops}
\end{table*}

In the following, we first define the scope of our semantic parser with the definition of \DBTalk, our formal target language.  We then describe the natural language sentences we synthesize with (1) canonical templates to cover all the possible queries and (2) generic query templates to provide linguistic variety. 

\iffalse
We propose to capture this variety in a rich general grammar of questions. 
Given a database, previous work by Wang et al.~\cite{overnight} proposes a general grammar that captures just set (1), and focuses almost exclusively on the join operation; they rely on paraphrasers to provide the varieties in both (2) and (3).  
 % Not only is this expensive, the coverage is very poor.
Our general grammar is larger and captures the variety along all three axes, to the point that we no longer need to rely on as much paraphrasing. This reduces cost and improves accuracy.
\fi
\input{sections/query-language}

\subsection{Canonical Templates}

To associate \DBTalk constructs with natural language, \SQA uses the previously proposed concept of \textit{templates}~\cite{geniepldi19}.
Templates are production rules mapping the grammar of natural language to a \textit{semantic function} that produces the corresponding code. 
Formally, a template is expressed as:
\begin{align*}
\textit{nt} := \left[v : \textit{nt}~~\vert~~\text{literal}\right]^+ \Rightarrow \textit{sf}
\end{align*}
The non-terminal \textit{nt} is produced by expanding the terminals and non-terminals
on the right-hand side of the $:=$ sign.
The bound variables $v$ are used by the semantic function \textit{sf} to produce the corresponding code.

For each operator in \DBTalk, we can construct a \textit{canonical template} expressing that operator in natural language.
The main canonical templates are shown in Table~\ref{table:db-ops}. The table omits logical connectives such as ``and'', ''or'', and ``not'' for brevity.
These canonical templates express how the composition of natural language is reflected in the composition of corresponding relational algebra operators to form complex queries.

With the canonical templates, we can cover the full functionality of \DBTalk, and thus
the full span of questions that the system can answer. However, these synthesized sentences do not reflect how people actually ask questions. In the next section, we discuss how we can increase the
variety in the synthesized set with a richer set of generic templates.

\iffalse
\TODO{REWRITE}
Two types of questions are commonly asked in natural language: search questions and information questions. 
Search questions retrieve records from the database based on a certain criteria, while information questions
get properties of certain records.
These two types of questions map to basic relational algebra operations.
A search question maps to a selection operation or a join operation (depending on if the criteria uses fields in one or multiple table).
A search question may also require sorting, indexing, slicing to present the search results.
An information question maps to a projection operation, extracting a specific field of a particular database row.
Both selection and projection can be applied to either existing fields or computed ones. 
Examplef on how relational algebra operations are used in natural language are shown in Table~\ref{table:db-ops}.

In practice, we find search questions to be more common for real-life database questions 
(as shown in Section~\ref{sec:experiments}).
Search questions also present more in natural language since people can naturally compose multiple criteria
in a single question.
For example, people can ask ``find me a 5-star Italian restaurants within 10 miles'' which includes 3 different criteria: rating, cuisine, and distance.
\fi

\iffalse
\begin{table}
\caption{Relational algebra operations in natural language.}
\small
\begin{tabular}{c|c|l}
\toprule
{\bf Type} & {\bf Operator} & {\bf Example} \\
\midrule
\multirow{2}{*}{Search}      & filter      & What is a <restaurant> that <serves Italian food>? \\ 

                             & join        & What is a <restaurant> that <has been reviewed by Bob>? \\
\hline
\multirow{3}{*}{Information} & projection  & What is <the kind of food served> by <McDonald's>? \\
                             & count       & How many <reviews> does <McDonald's> have? \\
                             & aggregation & how many <McDonald's> are there? \\
\bottomrule
\end{tabular}
\label{table:db-ops}
\end{table}
\fi

\subsection{Generic Query Templates}

\paragraph{Sentence Types}
Let's start with the concept of sentence types. In English there are four types: declarative, imperative, interrogative, and exclamatory. In \QandA, we care about declarative (``I am looking for {\em object}''), imperative (``Search for {\em object}'') and interrogative (``What is {\em object} ?'').
We have generic query templates to generate all these three different sentence types. 
Table~\ref{table:question_types2} shows examples for imperative and interrogative queries. 

Based on the type of object being queried, different interrogative pronouns can be used, in lieu of the generic ``what''.
% ``Who, what, where, when, why'' are 5 common pronouns in real life. Ignoring ``why'', which is not typically answered with a database, the rest are all mapped to the ``what'' questions in relational algebra. 
``Who'' maps to ``what is the person that''; ``where'' maps to ``what is the location of''; ``when'' maps to ``what is the time that''.   The distinction between persons, animals/inanimate objects, locations, and time is so important to humans that it is reflected in our natural language.  To create natural-sounding sentences, we create generic query templates for these different ``W''s and select the one to use according to the declared types of the fields in sentence synthesis. 

In addition, a question can also include available choices to make it a {\em choice question}, where the answer should be selected in the given candidates. 
A full sentence can also be turned into a {\em yes-no question}, to verify if the statement is true.
Empirically, we found these two types of questions to be much less common in the domains we experiment on. 
The templates for them are left for future work. 

 
\paragraph{Referring To Fields}
We are interested in questions asking about facts in a database.
A fact is stored as a field that connects an entity (a row in a table) to a value. 
In English, each fact can be expressed as a statement that either starts with the entity (forward direction) or the value (reverse direction). 
We found that how a field can be referred to in a statement exhibits great variety in natural language.
It can be described using a phrase that belongs to one of 11 different parts of speech, as shown in Table~\ref{table:question_types2}. 
We distinguish between noun phrases that describe what the subject has (has-a noun phrase) vs. what the subject is (is-a noun phrase).

For each statement, we can construct a question to query either the subject or the object (Table~\ref{table:question_types2}). 
If the part of the statement being asked is the entity in the table, the question maps to a selection operation.
Otherwise, it maps to a projection operation. 
For example, suppose we are interested in finding Stanford employees (a selection on the ``Person'' table). 
We can ask ``search for a person employed by Stanford'', ``who is employed by Stanford'', or ``who works at Stanford?''.
Similarly, if we are interested in finding where a person works (a projection on the ``worksFor'' field of the ``Person'' table), we can ask ``what is the employer of Bob?'', ``what company employs Bob?'', or ``what company has Bob as employee?''.

We have generic queries to refer to fields using all the different parts of speech.
In addition, some POS can also be used in a shorter phrase in a more natural way.
For example,
``has-a'' noun phrases can be used in a ``with'' phrase, such as ``person with Stanford as the employer''.
``Is-a'' noun phrases, on the other hand, can replace the subject directly as ``an employee of Stanford'' without mentioning ``person''.
Adjective phrases can be placed in front of the subject directly, such as ``Chinese person'' (Table~\ref{table:question_types2}). 


\iffalse
In total, we identified six POS categories that cover most of the ways fields are queried,   
as shown in Table~\ref{table:question_types2}. 
%Note that these POS are categorized based on how they can be used in natural language synthesis instead of parsing. 
We distinguish between noun phrases that describe what the subject has (has-a noun phrase) vs. what the subject is (is-a noun phrase).
We also distinguish, for each POS, whether the relationship in natural language matches the direction in which it is expressed in the database, or whether it is reversed.
\fi


\iffalse
\paragraph{Interrogative Pronouns}
Based on the type of object being queried, different interrogative pronouns can be used, in lieu of the generic ``what''.
% ``Who, what, where, when, why'' are 5 common pronouns in real life. Ignoring ``why'', which is not typically answered with a database, the rest are all mapped to the ``what'' questions in relational algebra. 
``Who'' maps to ``what is the person that''; ``where'' maps to ``what is the location of''; ``when'' maps to ``what is the time that''.   The distinction between persons, animals/inanimate objects, locations, and time is so important to humans that it is reflected in our natural language.  To create natural-sounding sentences, we create generic query templates for these different ``W''s and select the one to use according to the declared types of the fields in sentence synthesis. 

\Red{
\paragraph{Question Types}
A statement sentence is composed by two main parts - the subject and the predicate.
A predicate contains a verb, and optionally objects and complements. 
%Both subjects and objects can be qualified by an adjective or adjective equivalent, and verbs can be qualified by an adverb or adverb equivalent. 
Each of these components of a sentence can be asked by a question, as shown in Table.\ref{table:question_types}.
Which component is asked decides what database operation is needed for the query: 
asking a component related to property maps to projection operation, while asking a component related to the domain subject maps to selection operation.

% discussion on different parts of speech?

}
\fi

\begin{table*}
\caption{Example query constructions for the ``worksFor'' and ``nationality'' fields of the ``Person'' table}
\fontsize{7.7}{10}\selectfont
\setlength{\tabcolsep}{1.2pt}
\begin{tabular}{llll}
\toprule
{\bf Part-of-Speech} & {\bf Statement} & \bf Selection & \bf Projection\\
\midrule
base form       & The \Red{employer} of \Green{Bob} is \Blue{Stanford}. & \Green{Who} is a \Green{person} with \Red{employer} equal to \Blue{Stanford}?      & \Blue{What} is the \Red{employer} of \Green{Bob}? \\
                &                                   & Search for a \Green{person} with \Red{employer} equal to \Blue{Stanford}.  & Search for the \Red{employer} of \Green{Bob}.  \\
\toprule
fwd. has-a noun & \Green{Bob} has \Blue{Stanford} \Red{as the employer}. & \Green{Who} has \Blue{Stanford} \Red{as the employer}?                  & \Blue{What company} does \Green{Bob} have \Red{as the employer}? \\
                &                                   & Search for a \Green{person} with \Blue{Stanford} \Red{as the employer}. & Search for the \Blue{company} that \Green{Bob} has \Red{as the employer}. \\
\midrule
fwd. is-a noun  & \Green{Bob} is \Red{an employee of} \Blue{Stanford}.   & \Green{Who} is \Red{an employee of} \Blue{Stanford}?                    & \Blue{What company} is \Green{Bob} \Red{an employee of}? \\
                &                                   & Search for \Red{an employee of} \Blue{Stanford}.                & Search for the \Blue{company} that \Green{Bob} is \Red{an employee of}. \\
\midrule
fwd. verb       & \Green{Bob} \Red{works for} \Blue{Stanford}.           & \Green{Who} \Red{works for} \Blue{Stanford}?                            & \Blue{What company} does \Green{Bob} \Red{work for}? \\
                &                                   & Search for a \Green{person} that \Red{works for} \Blue{Stanford}.        & Search for the \Blue{company} that \Green{Bob} \Red{works for} \\
\midrule
fwd. participle & \Green{Bob} is \Red{employed by} \Blue{Stanford}.      & \Green{Who} is \Red{employed by} \Blue{Stanford}?                       & \Blue{What company} is \Green{Bob} \Red{employed by}? \\
                &                                   & Search for a \Green{person} \Red{employed by} \Blue{Stanford}.   & Search for the \Blue{company} that \Green{Bob} is \Red{employed by}. \\
\toprule
rev. has-a noun & \Blue{Stanford} has \Green{Bob} \Red{as an employee}.  & \Green{Who} does \Blue{Stanford} have \Red{as an employee}?                & \Blue{What company} has \Green{Bob} \Red{as an employee}? \\
                &                                   & Search for a \Green{person} that \Blue{Stanford} has \Red{as an employee}. & Search for the \Blue{company} that has \Green{Bob} \Red{as an employee}. \\
\midrule
rev. is-a noun  & \Blue{Stanford} is \Red{the employer of} \Green{Bob}.  & \Green{Who} is \Blue{Stanford} \Red{the employer of}?                      & \Blue{What company} is \Red{the employer of} \Green{Bob}? \\
                &                                   & Search for a \Green{person} that \Blue{Stanford} is \Red{the employer of}. & Search for \Red{the employer of} \Green{Bob}. \\
\midrule
rev. verb       & \Blue{Stanford} \Red{employs} \Green{Bob}.             & \Green{Whom} does \Blue{Stanford} \Red{employ}?                            & \Blue{What company} \Red{employs} \Green{Bob}? \\
                &                                   & Search for a \Green{person} that \Blue{Stanford} \Red{employs}.            & Search for the \Blue{company} that \Red{employs} \Green{Bob}. \\
\midrule
rev. participle & \Blue{Stanford} is \Red{employing} \Green{Bob}.        & \Green{Who} is \Blue{Stanford} \Red{employing}?                            & \Blue{What company} is \Red{employing} \Green{Bob}? \\
                &                                   & Search for \Green{person} that \Blue{Stanford} is \Red{employing}.         & Search for the \Blue{company} \Red{employing} \Green{Bob}. \\
\hline
\hline
preposition     & \Green{Bob} is \Red{from} \Blue{China}. & \Green{Who} is \Red{from} \Blue{China} ?      & \Blue{Where} is \Green{Bob} \Red{from}?\\
                &                                          & Search for a \Green{person} \Red{from} \Blue{China}.  & Search for \Blue{where} \Green{Bob} is \Red{from} \\

\midrule
adjective       & \Green{Bob} is \Blue{Chinese}.     & \Green{Who} is \Blue{Chinese} ?      & - \\
                &                                   & Search for a \Red{Chinese} \Green{person}.  & -  \\
\bottomrule
\end{tabular}
\label{table:question_types2}
\end{table*}

\iffalse
\begin{table*}
\caption{Noun phrase construction and question forms (with examples from the Person domain).
In italics are the placeholders, which are replaced with either a reference to the table or a specific value.
The reference to the table can be a bare noun or itself a noun phrase.
In red is the part of the sentence that refers to the field, and in blue is the type of the field value. 
}
\small
\begin{tabular}{l|l|l|l}
\toprule
{\bf Part-of-Speech} & {\bf Noun-phrase form} & \bf Question form (selection) & \bf Question form (projection)\\
\hline
base form & \Red{employer} of \Green{\textit{person}} & what \Green{\textit{person}} has \Red{employer} equal to \textit{company} & what is the \Red{employer} of \Green{\textit{person}} \\
\hline
has-a noun (fwd) & \Green{\textit{person}} with \textit{company} \Red{as employer} & what \Green{\textit{person}} has \textit{company} \Red{as employer} & what \Blue{company} does the \Green{\textit{person}} have \Red{as employer} \\
has-a noun (rev) & \Blue{company} with \Green{\textit{person}} \Red{as employee} & what \Green{\textit{person}} the \textit{company} has \Red{as employee} & what \Blue{company} has \textit{person} \Red{as employee} \\
\hline
is-a noun (fwd) & \Green{\textit{person}} that is \Red{employee of} \textit{company} & what \Green{\textit{person}} is \Red{employee of} \textit{company} & what \Blue{company} is the \Green{\textit{person}} \Red{employee of} \\
is-a noun (rev) & \Blue{company} that is the \Red{employer of} \Green{\textit{person}} & what \Green{\textit{person}} is \textit{company} \Red{employer of} & what \Blue{company} is the \Red{employer of} \Green{\textit{person}} \\
%is-a noun (impl.) & \Green{\textit{person}} that is \textit{job title} & what \Green{\textit{person}} is \textit{job title} & \\
\hline
verb (fwd) & \Green{\textit{person}} that \Red{works for} \textit{company} & what \Green{\textit{person}} \Red{works for} \textit{company} & what \Blue{company} does the \Green{\textit{person}} \Red{work for} \\
verb (rev) & \Blue{company} that \Red{employs} \Green{\textit{person}} & what \Green{\textit{person}} does \textit{company} \Red{employ} & what \Blue{company} \Red{employs} \Green{\textit{person}} \\
\hline
passive verb (fwd) & \Green{\textit{person}} \Red{employed by} \textit{company} & what \Green{\textit{person}} is \Red{employed by} \textit{company} & what \Blue{company} is \Green{\textit{person}} \Red{employed by} \\
passive verb (rev) & \Blue{language} \Red{spoken by} \Green{\textit{person}} & what \Green{\textit{person}} is \textit{language} \Red{spoken by} & what \Blue{language} is \Red{spoken by} \Green{\textit{person}} \\
\hline
adjective & \textit{language} \Red{speaking} \Green{\textit{person}} & what \Green{\textit{person}} is \textit{language} \Red{speaking} & what \Blue{language} is \Green{\textit{person}} \Red{speaking} \\
%adjective (impl.) & \textit{company} \Green{\textit{person}} & what \Green{\textit{person}} is \textit{company} & \\
%\hline
%preposition (fwd) & \Green{\textit{person}} \Red{from} \textit{city} & what \Green{\textit{person}} is \Red{from} \textit{city} & what \Blue{city} is \Green{\textit{person}} \Red{from} \\
%preposition (rev) & \Blue{city} \Red{of} \Green{\textit{person}} & what \Green{\textit{person}} is \textit{city} \Red{of} & what \Blue{city} is \Red{of} \Green{\textit{person}}\\
\bottomrule
\end{tabular}
\label{table:question_types2}
\end{table*}
\fi

\iffalse
\begin{table*}
\caption{Example questions for restaurant domain.}
\small
\begin{tabular}{l|l|l|l}
\toprule
{\bf Statement} & {\bf Component to ask} & {\bf DB operation} & {\bf Question}\\
\hline
The restaurant serves Italian cuisine & Subject (``the restaurant'') & selection & Which restaurant serves Italian cuisine?\\
\hline
The restaurant serves Italian cuisine & Object (``Italian cuisine'') & projection & What cuisine does the restaurant serve?\\
\hline
The restaurant is located at Stanford & Complement (``at Stanford'') & projection & Where is the restaurant located at?\\
\hline
The restaurant allows smoking & Predicate (``allows smoking'') & projection & Does the restaurant allow smoking? \\
\hline
The restaurant is 5-star & Predicative (``5-star'') & projection & What is the rating of the restaurant? \\
\bottomrule
\end{tabular}
\label{table:question_types}
\end{table*}
\fi


{\renewcommand{\arraystretch}{0.9}
\begin{table}[tb]
\small
\caption{Type-specific comparison words.}
\vspace{-0.5em}
\label{table:type-comparisons}
\begin{tabular}{ll}
\toprule
\bf Type & \bf Comparative \\
\midrule
Time     & earlier, before, later, after \\
Duration & shorter, longer \\
Distance & closer, nearer, farther, more distant \\
Length & shorter, longer \\
Currency & cheaper, more expensive \\ 
Weight & lighter, smaller, heavier, larger \\
Speed & slower, faster \\
Temperature & colder, hotter \\
\bottomrule
\end{tabular}
\end{table}
}


\paragraph{Types and Measurements}
\iffalse
``Who, what, where, when, why'' are 5 common kinds of questions asked in real life. Ignoring ``why'', which is not typically answered with a database, the rest are all mapped to the ``what'' questions in relational algebra. 
``Who'' maps to ``what is the person that''; ``where'' maps to ``what is the location of''; ``when'' maps to ``what is the time that''.   The distinction between persons, animals/inanimate objects, locations, and time is so important to humans that it is reflected in our natural language.  To create natural-sounding sentences, we create generic query templates for these different ``W''s and select the one to use according to the declared types of the fields in sentence synthesis.  
\fi

The encoding of types in language carries over to measurements. Mathematical operators such as ``$a < b$'', ``$a > b$'', ``min'', ``max'' translate to different words depending on the kind of measurements. For example, for weight we can say ``heavier'' or ``lighter''. The list of type-specific comparison words is shown in Table~\ref{table:type-comparisons}. For each type, there are corresponding superlative words (``heaviest'', ``lightest'', etc.).
There is a relatively small number of commonly used measurements.  By building these varieties in the training data synthesis, we do not have to rely on manually annotated data to teach the neural networks these concepts. 

Types are also expressed in certain common, shortened question forms. For example, rather than saying ``what is the distance between here and X'', we can say ``how far is X''; the ``distance'' function and the reference point ``here'' are implicit. Similarly, instead of saying ``the restaurant with the shortest distance from here'', we can say ``the nearest restaurant''. These questions are sufficiently common that it is useful to include them in the generic set.

\iffalse
\begin{verbatim}
Length: shorter, longer, shortest, longest
Weight: lighter, heavier, lightest, heaviest
Time: earlier, later, earliest, latest
Cost: cheaper, more expensive, cheapest, most expensive
\end{verbatim}
\fi

\iffalse
\begin{table*}
\caption{Different part-of-speech for modifiers.}
\small
\begin{tabular}{l|l|l|l}
\toprule
{\bf Synthesis POS} & {\bf Example field} & {\bf Example phrase} & {\bf Example sentence}\\
\midrule
has-a noun phrase & alumniOf & degree from \# &  show me people who have a degree from X university\\
\hline
is-a noun phrase & alumniOf & alumni of \# & show me people who are alumni of X university\\
\hline
verb phrase & alumniOf & graduated from \# & show me people who graduated from X university  \\
\hline
passive verb phrase & alumniOf & educated at \# & show me people who are educated at X university\\
\hline
adjective phrase & servesCuisine & \# & show me restaurants which is Italian.\\
\hline
preposition phrase & geo & in \# & show me restaurants which is in X city.\\
\bottomrule
\end{tabular}
\label{table:pos}
\end{table*}
\fi
\iffalse
\TODO{Make into a table, add examples, and description}
\begin{verbatim}
Implicit subject: <property>
Adjective:        <property><subject>
                  <argmax/argmin><subject>
Phrase: With <property> <operator> <value>
        <passive-verb><value>
Clauses with variety in types of subject: which have/which are, who are, whose 
             adjective, 
             passive voice, 
             implicit "fields",  
             argmax table
\end{verbatim}
\fi


\paragraph{Connectives}
In natural language, people use connectives to compose multiple clauses
together, when they wish to search with multiple filters or joins.
Clauses are normally connected with an explicit connective 
such as ``and'', ``but''. 
However, the connective can also be implicit, when composing natural short phrases 
based on its part-of-speech category.

The different POS categories and connectives give modifiers great varieties in natural language.
By taking into account what modifiers are used by two phrases, we can combine them in
a natural way. % Fig.~\ref{fig:connectives} shows some example of possible combinations.
For example, multiple adjective phrases can be concatenated directly: 
people say ``5-star Italian restaurants'' rather than ``5-star and Italian restaurants''.
Similarly, a phrase that uses the adjective ``Chinese'',
can be combined with the ``has-a'' noun phrase ``4 stars'' using the connective
``with'', to form ``Chinese restaurants with 4 stars''.
% Conversely, if
%two ``has-a'' noun phrases, such as ``Chinese food'' and ``4 stars'' are
%connected with ``and'', to form ``restaurants that have Chinese food and 4 stars''.

%\TODO{How to add multiple filters and joins together in natural language?}
\iffalse
\subsection{Variety in Domain-Specific Ontology}
Each domain has its own variety in natural language that cannot be generalized.
The subject can be referred by varies synonyms, and each field can be used in different POS categories.
As shown in Table~\ref{table:pos}, the same property ``almuniOf'' can used in four 
different parts of speech. 
For the same POS category, there can also be different phrases to use. 

These phrases do not necessarily have to be synonyms in general,
but they share the same meaning in the specific domain.
This type of knowledge are not generalizable across different domains.
Thus, it's important to allow domain expert to supply the domain-specific ontology
in training data synthesis, to reach a good coverage of an unseen domain. 
\fi

\iffalse

Templates corresponding to the generic question families (Section~\ref{}) are written by hand, and map natural language compositional constructs to formal language operators.
Many sentences can be covered with a combination of generic templates and domain-specific canonical forms, such as:
\begin{tabbing}
12345678901234\=1234\=\kill
\>table $:=$ $t : \text{table}$ ``that'' $p : \text{vb}$ $v : \text{value}$ \\
\>\>$\Rightarrow t, \text{contains}(p, v)$
\end{tabbing}
This template can generate ``hotel that offers free parking''.
In this case, the table is ``Hotel'', and the field is ``amenityFeature'' with has canonical form ``offers'' in the VB (verb) category.
Templates rely on the type system of \DBTalk to form sentences that are meaningful and map to correct queries. The semantic function
in each template verifies that the \DBTalk query has the correct type, and the type is appropriate for the corresponding natural
language (e.g. a generic template using ``less than'' must be used with a field of comparable type).
%For example, in the following template, only fields of comparable type can be used:
%\begin{tabbing}
%123\=1234\=\kill
%\>table $:=$ $t : \text{table}$ ``whose'' $p : \text{npp}$ ``is less than'' $v : \text{value}$ \\
%\>\>$\Rightarrow t, p \le v$
%\end{tabbing}
%The template would generate ``restaurants whose rating is less than 3'', but it would not generate
%``restaurants whose cuisine is less than Italian'', as the latter would not typecheck.
\fi

\subsection{Supplying Domain-Specific Knowledge}
The domain-specific information necessary to generate questions is provided by the developer
in form of annotations on each field. Table~\ref{table:canonicals} shows examples of annotations for 3 fields
in the database. The developer is expected to provide as many variations as possible of each property.
Even for the same POS category, there may be alternatives using different words.
For example, ``alumniOf'' can have two different verb phrases ``studied at'' and ``attended''.
The examples in this table also show that not every field can be referred to using the 6 POS modifiers.  
For restaurants, 
we can say ``has French food'', ``serves French food'', ``French restaurant'', but not
``restaurant is a French'', ``served at French'', or ``a restaurant of French''. 
Similarly, for ratings, we can say ``has 5 stars'', ``rated 5 stars'', ``5-star restaurant'', but not ``restaurant is a 5 rating'', ``restaurant rates 5'', or a ``restaurant of 5 stars''.  
We rely on the domain expert to annotate their fields with appropriate phrases for each POS category.  

\input{sections/table-pos}

\subsection{Template-Based Synthesis}

To synthesize data for the neural semantic parser, \webqa uses the Genie template-based 
algorithm~\cite{geniepldi19}, with our curated set of about 600 generic query templates. 
Genie expands the templates by substituting the non-terminals with the previously generated
derivations and applying the semantic function. Because the expansion is exponential, only a limited
fraction of the possible combinations are sampled. The expansion continues recursively, up to a configurable depth. 

A small portion of the synthesized data is paraphrased by crowdsource workers.
Both the synthetic and paraphrased sets are then augmented by replacing the field values with 
the actual values in the knowledge base. 
This allows us to expose more real values to the neural network
to learn how they match to different fields.

Because synthesized data is used in training, \webqa training sets cover a lot more questions that previous methods based
only on paraphrasing. \webqa does not need to rely on the distribution on sentences in the training set to match the test set.
Instead, it only needs to generalize minimally from sentences that are present
in the training set. As long as the training set has good coverage of real world questions, this ensures high accuracy.
Additionally, developers can refine their skills with more templates.

\iffalse
\TODO{move down} The pipeline to get the final training examples is shown in Figure~\ref{fig:genie}.

\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{./figures/genie-diagram.pdf}
\caption[]{Training data synthesis pipeline.}
\label{fig:genie}
\Description{}
\end{figure}
\fi

